Thermoplasmonics under optically coupled regime: A Numerical Study of Dimers, Nanolenses, and Switchable Clusters

The management of thermal effects in plasmonic nanostructures is frequently viewed as a detrimental waste rather than a useful, controllable entity. We show that optical coupling of plasmonic nanoparticles enables precise spatiotemporal control over nanoscale heating. Through numerical investigation of experimentally-achievable systems from individual nanoparticles and dimers to nanolenses and switchable clusters, we demonstrate how plasmon hybridization and near-field coupling dictate the magnitude and spatial distribution of temperature. Our results highlight the critical role of polarization and gap distance in tuning the thermal output of dimers, the ability of a trimer nanolens to focus heat into a sub-diffraction volume, and the pronounced thermal difference in a switchable nanoparticle cluster. This work establishes a framework for designing advanced thermoplasmonic systems where heat is not merely a detriment, but a dynamically controllable element for applications in catalysis, health, or active photonic devices.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
